Knowledge Tracing for Complex Problem Solving: Granular Rank-Based Tensor Factorization

Knowledge Tracing (KT), which aims to model student knowledge level and predict their performance, is one of the most important applications of user modeling. Modern KT approaches model and maintain an up-to-date state of student knowledge over a set of course concepts according to students' historical performance in attempting the problems. However, KT approaches were designed to model knowledge by observing relatively small problem-solving steps in Intelligent Tutoring Systems. While these approaches were applied successfully to model student knowledge by observing student solutions for simple problems, they do not perform well for modeling complex problem solving in students.M ost importantly, current models assume that all problem attempts are equally valuable in quantifying current student knowledge.However, for complex problems that involve many concepts at the same time, this assumption is deficient. In this paper, we argue that not all attempts are equivalently important in discovering students' knowledge state, and some attempts can be summarized together to better represent student performance. We propose a novel student knowledge tracing approach, Granular RAnk based TEnsor factorization (GRATE), that dynamically selects student attempts that can be aggregated while predicting students' performance in problems and discovering the concepts presented in them. Our experiments on three real-world datasets demonstrate the improved performance of GRATE, compared to the state-of-the-art baselines, in the task of student performance prediction. Our further analysis shows that attempt aggregation eliminates the unnecessary fluctuations from students' discovered knowledge states and helps in discovering complex latent concepts in the problems.

==> 2_related.tex <==
%  Researchers have been investigating mathematical and computational models to tackle the KT task since the 1990s. 
 Various approaches, which range from probabilistic models to deep neural networks, have been developed over the past two decades to tackle the KT task. 
 The Bayesian knowledge tracing (BKT) model was proposed in \cite{corbett1994knowledge} during the 1990s. 
 It models the knowledge states of KCs using one HMM for each individual KC. 
 Many variants of BKT have been proposed to improve the model by considering forgetting power\cite{hawkins2014learning}, skill dependency \cite{kaser2017dynamic}, and personalization \cite{yudelson2013individualized}, among others.  
 Learning factors analysis (LFA) and performance factors analysis (PFA) were proposed in the 2000s, which incorporate student ability into the logistic regression model, to deal with the issue of multiple knowledge components. 
 However, they cannot deal with the inherent dependency among KCs and require prior knowledge of the overall domain model - the association between knowledge components and learning materials. 
 Some latent factor approaches \cite{thai2012factorization}\cite{lan2014sparse}\cite{sahebi2016tensor}\cite{zhao2020modeling} have been investigated in recent years to overcome this limitation. 
 Lan et al. \cite{lan2014sparse} proposed a sparse factor analysis framework for learning and content analytics. 
 Sahebi et al. \cite{sahebi2016tensor} proposed a tensor factorization method to explicitly model students' learning process by assuming a strictly monotonic increasing learning gain.     
 Zhao et al. \cite{zhao2020modeling} leverage the multiview tensor factorization method for modeling student knowledge using multiple learning resource types.  
 Deep learning models, such as DKT\cite{piech2015deep} and DKVMN\cite{zhang2017dynamic}, have recently been introduced into the KT domain, as they have enough capacity to automatically learn the inherent relationships and do not require explicit labels on the concept level as well.
 However, a deep learning-based model is not always the best choice for KT problem in terms of data efficiency, interpretability, and prediction accuracy \cite{gervet2020deep} \cite{khajah2016deep} \cite{wilsonback}. 


==> 3_preliminary.tex <==
% \subsection{Notation}

% \begin{table*}[!ht]
% \vspace{-5pt}
% \centering

% \begin{center}
% \begin{tabular}{|c|c|} 
%  \hline
%  $\mathbold{X}, \mathbold{Y}, \mathbold{T}, \Tilde{\mathbold{T}}, \Tilde{\mathbold{K}}$ & denote 3-mode tensors   \\ 
%  \hline
%  $\mathcal{M}, \mathcal{K}, \mathcal{C}, \mathcal{N}, \mathcal{T}, \Tilde{\mathcal{T}}$ & denote dimensions \\
%  \hline
%  $S, Q, W$ & denote matrices \\ 
%  \hline
%  $\omega_{u,t,i}, x_{u,\Tilde{t},i}$, $y_{u,t,i}, q_{c,i}, b_u, b_i, \mu$  & denote scalar values.\\
%  \hline
% \end{tabular}
% \end{center}

% \caption{Notations}
% \label{table:notation}
% \end{table*}



% \subsection{Tensor Factorization}

% \subsection{Learning Analytics and Content Analytics via Adaptive Granularity Rank-based Tensor Factorization}
% In this paper, we adopt the idea of multiview knowledge model with rank-based tensor factorization \cite{zhao2020modeling} and apply to our student and domain knowledge modeling on single view dataset.
% Notice that, our recommendation method could be applied to other student and domain knowledge modeling methods, especially with the general linear interactions.
% There are some advantages of RBTF that make it well suited to our proposed recommendation method. 
% First, RBTF is capable to model student knowledge interactively and sequentially. 
% Second, students' knowledge increasing and forgetting patterns are well-modeled, which leads to consistent student performance prediction as well as interpretable knowledge dynamic of change. The details of RBTF model will be illustrated below.

% Given a tensor $\mathbf{X}\in [0,1]^{|U|\times T \times |I|}$ storing student sequential interaction records, entry $x_{u,t,i}$ represents the $u^{th}$ student's grade on $i^{th}$ question at time or attempt $t$. $U$ is the set of students, $I$ is the set of learning contents or questions, $T$ denotes the total number of time stamps. RBTF is to factorize the students' interaction records and predict a student's grade as $
%     \hat{x}_{u,t,i} = \sigma(\mathbf{s}_{u,t} \cdot \mathbf{q}_{i} + b_{u} + b_{t} + b_i)
% $,
% where $\mathbf{s}_{u,t}$ represents the student knowledge embedding of student $u$ at time $t$, $\mathbf{q}_{i}$ denotes by the latent feature vector or concept embedding of question $i$, and $b_u$, $b_t$, and $b_i$ are biases for student $u$, time $t$, and question $i$, respectively.
% In order to learn the model parameters ($\mathbf{s}_{u,t}, \mathbf{q}_i, b_u, b_t,$ and $b_i$), RBTF aims to minimize the regularized squared error:
% \begin{equation}
%     \begin{split}
%     \mathcal{L}_1 &=  \sum_{u,t,i \in \Omega_{obs}} \left(x_{u,t,i} - \hat{x}_{u,t,i} \right)^{2} + \lambda_t \|S_t\|^2_F  \\
%     & \ \ \ \ \ \ \ \ \ \ \  + \lambda_b \left(\|b_u\|^2 + \|b_t\|^2 + \|b_i\|^2 \right)
%     \end{split}
%     \label{eq:loss_1}
%     % \mathop{\textbf{minimize}}_{\mathbf{p}_u, \mathbf{T}_t, \mathbf{q}_i, b_u, b_t, b_i} 
% \end{equation}
% where the set $\Omega_{obs} \subseteq \{1, \cdots, |U|\} \times \{1, \cdots, T\} \times \{1, \cdots |I|\}$ contains the indices associated with observed graded student response data. Furthermore, RBTF also assumes that students' knowledge on specific concepts always increase after interaction with those concepts in a specific question, and their scores at attempt $t+1$ on question $i$ are expected to be more than their scores at attempt $t$, that is 
% $
%     \mathbf{s}_{u, t} \cdot \mathbf{q}_i \leq  \mathbf{s}_{u, t+1} \cdot \mathbf{q}_i
% $.

% To increase the interpretability, the question latent feature vector $\mathbf{q}_{i}$ is enforced to be non-negative and summed to one, which could be achieved by clipping and normalizing the values in $\mathbf{q}_i$.
% Therefore, the objective of RBTF method could be formulated as 
% \begin{equation}
%   \begin{split}
%     \mathop{\textbf{minimize}}_{\mathbf{s}_{u,t}, \mathbf{q}_i, b_u, b_t, b_i} \mathcal{L} &= \mathcal{L}_1 + \omega \mathcal{L}_2 \\
%     \text{subject to}\ \ &q_{k,i} \geq 0 \ \ \  \forall k, i\\
%     & \sum_{k} q_{k,i} = 1.
%   \end{split} 
% \end{equation}
% where $\omega$ is the trade-off parameter for penalty term $\mathcal{L}_2$:
% \begin{equation}
%     \mathcal{L}_2 = -\sum_{j=1}^{t-1} \sum_{u,i} \log \left( \sigma \left( \mathbf{S}_{u, t} \cdot \mathbf{q}_i -  \mathbf{S}_{u, j} \cdot \mathbf{q}_i \right) \right), 
% \end{equation}
% in which $\sigma$ represents the sigmoid function. A local minimal could be achieved by using stochastic gradient descent, and interpretable student and concept embeddings could be obtained and validated. 


% \subsection{Normalized Discounted Cumulative Gain}
% For top-$k$ items recommendation, the ranking of those $k$ items determines the performance of the recommender system, since it is more useful to have the highly relevant items appear earlier in the ranking list. 
% One of the most commonly used ranking metrics in search engines or recommender systems is the \textit{normalized discounted cumulative gain (nDCG)}:
% \begin{equation}
%     \operatorname{nDCG} =\frac{1}{\mathcal{Z}} \sum_{j=1}^{k} \frac{2^{r_{j}}-1}{\log _{2}(j+1)}
% \end{equation}
% where $r_j$ is the real rating or relevance of the item shown at ranking position $j$, and $\mathcal{Z}$ is the normalization factor making the score of the optimal ranking to $1$ such that $0 \leq nDCG \leq 1$. In other words, $\mathcal{Z}$ is simply the value of discounted cumulative gain of optimal ranking.  
% In sequential recommendation systems, nDCG is generally used in online evaluations, which requires users' rating information in an interactive manner.
% However, in educational domain, the rating annotation for questions is irrelevant. %, except the logged student interaction records.
% Hence, we have to come up with a new approach for evaluation of educational recommender systems. 

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

